Train Unit Shunting and Servicing: a Real-Life Application of Multi-Agent Path Finding

In between transportation services, trains are parked and maintained at shunting yards. The conflict-free routing of trains to and on these yards and the scheduling of service and maintenance tasks is known as the train unit shunting and service problem. Efficient use of the capacity of these yards is becoming increasingly important, because of increasing numbers of trains without proportional extensions of the yards. Efficiently scheduling maintenance activities is extremely challenging: currently only heuristics succeed in finding solutions to the integrated problem at all. Bounds are needed to determine the quality of these heuristics, and also to support investment decisions on increasing the yard capacity. For this, a complete algorithm for a possibly relaxed problem model is required. We analyze the potential of extending the model for multi-agent path finding to be used for such a relaxation.

==> plan.tex <==
Title suggestions:
\begin{itemize}
    \item Train Unit Shunting: a Real-Life Application of Multi-Agent Path Finding
\end{itemize}

Introduction:
\begin{itemize}
    \item TUSP informal introduction -- routing part of problem; importance of problem (and similar to other problems)
    \item TUSP is not yet solved; algorithmically challenging
    \item similarity to MAPF
    \item main question: how to use MAPF algorithms for TUSP
    \item our contributions: identifying differences and presenting these as step-wise extensions of MAPF, benchmark data?
\end{itemize}



For literature review:
\begin{itemize}
    \item detailed description of TUSP practice (see introduction of thesis Roel, en anderen): doel: explain train shunting problem to laymen
    \item TUSP literature (e.g. Kroon et al.) -- matching
    \item difference from MAPF and task allocation: in TUSP tasks are maintenance and cleaning and come with the train (so allocation is not part of the problem)
\end{itemize}

For model section(s):
\begin{itemize}
    \item basic graph model for MAPF
    \item each of extensions from conclusions
    \item maybe as MILP?
\end{itemize}

For analysis/discussion:
\begin{itemize}
    \item does an optimal solution provide a bound on the real world feasibility? (e.g. is the model itself a relaxation?)
\end{itemize}


For conclusions:
\begin{itemize}
    \item matching is part of the problem -- similarity to colors/types of agents
    \item abstract model for long tracks (corridors) -- (when) is this necessary, what are straightforward alternatives (e.g. discretisation such as in grids) and their (dis)advantages (first assume single-units only)
    \item "kop maken": extra costs for changing direction
    \item parking only on certain tracks
    \item algorithms need to be able to deal with multiple way-points (possibly with tasks)
    \item sometimes there are multiple options for a waypoint (e.g. multiple tracks where maintenance can be done)
    \item ``way points'' are tasks with different durations
    \item more detailed timing; e.g., braking, speeding, maximum speeds, safety constraints on crossings
    \item objective: is makespan or sum of path costs the most relevant objective?  number of train drivers required seems a better one, but these are not in our model (currently), so maybe: number of simultaneous movements, or number of ``startups``
\end{itemize}

For future work:
\begin{itemize}
    \item apart from extending MAPF algorithms to deal with the above (and comparing them), we think research in this direction would benefit from...
    \item simulator
    \item couple/decouple train units from/into longer trains
    \item allocation of personnel (including walking times, constraints on working/driving times)
    \item introducing disturbances
    \item relevant for practice: interactive problem solving (mixed-initiative): not everything can always be modeled and/or given to the solver as input
\end{itemize}
